Revealing Vulnerabilities of Neural Networks in Parameter Learning and Defense Against Explanation-Aware Backdoors

Explainable Artificial Intelligence (XAI) strategies play a crucial part in increasing the understanding and trustworthiness of neural networks. Nonetheless, these techniques could potentially generate misleading explanations. Blinding attacks can drastically alter a machine learning algorithm's prediction and explanation, providing misleading information by adding visually unnoticeable artifacts into the input, while maintaining the model's accuracy. It poses a serious challenge in ensuring the reliability of XAI methods. To ensure the reliability of XAI methods poses a real challenge, we leverage statistical analysis to highlight the changes in CNN weights within a CNN following blinding attacks. We introduce a method specifically designed to limit the effectiveness of such attacks during the evaluation phase, avoiding the need for extra training. The method we suggest defences against most modern explanation-aware adversarial attacks, achieving an approximate decrease of ~99\% in the Attack Success Rate (ASR) and a ~91\% reduction in the Mean Square Error (MSE) between the original explanation and the defended (post-attack) explanation across three unique types of attacks.

==> sec/2_related_old.tex <==
\section{Related Works}
\label{sec:related}
Although numerous seminal papers have demonstrated that XAI methods can be employed to detect adversarial model fooling and sanitize inputs, XAI itself is not immune to these attacks \cite{chou2020sentinet,Subramanya2018FoolingNI}. This vulnerability presents a significant challenge in safeguarding models against adversarial attacks. The ongoing research in this field underscores the importance of developing robust and secure XAI methods that can withstand such sophisticated threats.

In the burgeoning field of adversarial attack defense, a plethora of methodologies has been proposed in recent literature. These strategies can be broadly classified into three categories: enhancements to the training process, modifications to the network activation, and implementation of supplementary models or metrics for bolstered adversarial robustness.

\citet{chen2019robust} proffered an innovative approach termed as robust Integrated Gradient Attribution that incorporates regularisation loss of attribution into the training loss of the neural network. Despite its novelty, this method does not offer a guarantee against future attacks as malevolent entities could subtly alter model parameters to manipulate explanations.

Taking a similar route but with a different strategy, \citet{tang2022defense} introduced Adversarial Training on EXplanations (ATEX), a novel training scheme designed to enhance the internal explanation stability of a model irrespective of the specific explanation method deployed. ATEX sidesteps the inclusion of second-order derivatives in optimization by solely imposing constraints on model predictions.

In line with these advancements, \citet{joo2023towards} propose an alignment regularization for the training objective function of networks to generate robust attributions. This method amalgamates both $L_2$ and cosine distance-based criteria as regularization terms, thereby harnessing their respective advantages in aligning local gradients. Similarly, \citet{wicker2022robust} leverage constraint relaxation techniques from non-convex optimization in neural network training. Their method develops an upper-bound for the largest change an adversary can make to a gradient-based explanation via bounded manipulation of either input features or model parameters.
**Incorporation of Additional Models or Metrics for Enhanced Robustness:**

\citet{rieger2020simple} presented an efficacious defense against adversarial attacks on neural networks by aggregating multiple explanation methods. This strategy fortifies the network against manipulation but could potentially introduce noise generated by each individual explanation method.

\citet{lakkaraju2020robust} proposed surrogate model training for generating robust explanations by minimizing an objective function that utilizes adversarial samples during the training of the explainer. The proxy explainer thus discerns which features are most consequential to the original classifier.

In a similar vein, \citet{yuyou2022mif} propose Median Test for Feature Attribution (MeTFA) as a tool to quantify uncertainty and bolster stability of explanation algorithms with theoretical guarantees. MeTFA is method-agnostic and can be applied to any feature attribution method. It introduces noise into input images and generates multiple explanations corresponding to each noisy instance.

\citet{vrevs2022preventing} advocated for improved sampling that employs data generators to learn the training set distribution and generate new perturbation instances more akin to the training set. They demonstrated that this enhanced sampling bolsters LIME and SHAP’s robustness.

\citet{dombrowski2022towards} and \citet{dombrowski2019explanations} proposed training with weight decay, smoothing activation functions, and minimizing the Hessian of the network weights. They identified that a large curvature of the network’s decision function is a significant contributor to this unexpected vulnerability. To mitigate this, they propose $\beta$-smoothing of explanations which calculates an explanation using a network where relu non-linearity is supplanted by softplus with a diminutive $\beta$ parameter to smooth principle curvatures.

Most existing literature focuses on addressing challenges through new training strategies, ensembling, proxy networks, or smoothing activation functions, with only limited research examining the effect of backdoor attacks on the learning parameters of neural networks. Instances of such research include that which investigates which layer weights are most affected by attacks and the patterns thereof. In this study, we analyze the three most recent state-of-the-art loss optimization based attacks, training them with two distinct loss functions. After training multiple weights on a specific network with a variable seed rate and subjecting them to attacks, we assess the weight alterations across varying layers. This analysis serves as the foundation for our proposed solution, CFN, which, despite its simplicity, is remarkably effective.

We additionally juxtapose our method with Softplus smoothed training\cite{dombrowski2022towards}, as presented in prior research. We note that the attack under our consideration is of recent development and the previous solution proved to be ineffective\cite{noppel2023disguising,doan2020februus}. Indeed, to evaluate the effectiveness of our method, we deem it necessary to compare our predictions and explanations with those of an unattacked model.


==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/draft.tex <==

The function `normalize_tensor(X)` you provided is implementing a process known as Batch Normalization for a 3D tensor (image) across the height and width dimensions. 

Here is the mathematical representation of the function:

Given a tensor `X` with dimensions (M, C, H, W) where C is the number of channels, H is the height and W is the width of the tensor.
MC
1. Compute the mean across the height and width dimensions:

    μ_c = 1/(H*W) Σ (X_c[m, i, j]) for all m in M, i in H and j in W,

2. Compute the variance across the height and width dimensions:

    σ²_c = 1/(H*W) Σ ((X_c[m, i, j] - μ_c)²) for all m in M i in H and j in W

3. Normalize the tensor:

    X_hat_c = (X_c - μ_c) / sqrt(σ²_c + ε)

where:
- μ_c is the mean of the elements of X across the height and width dimensions.
- σ²_c is the variance of the elements of X across the height and width dimensions.
- ε is a small number added for numerical stability (to avoid division by zero), in this case, ε = 1e-5.
- X_hat_c is the normalized tensor.

==> sec/method_dropout.tex <==
\subsection{Predictive Log-likelihoo}

Given a dataset $X$, $Y$ and a new data point $x^*$, we can estimate the likelihood of potential output values $y*$ through the predictive probability $p(y^*|x^*, X, Y)$. The log of the predictive likelihood informs how aptly the model fits the data, where higher values suggest a better fit of the model. The predictive log-likelihood can be estimated by using Monte Carlo integration of equation \ref{mcequation} with $T$ terms.

\begin{align*}
\log p(y^{*}| x^{*}, X, Y) & = \log \int p(y^{*}|x^{*}, w)p(w|X, Y) \, dw \\
& \thickapprox \log \int p(y^{*} |x^{*}, w)q(w)dw 
\\ & \thickapprox \log \bigg {(} \frac{1}{T}\sum_{t =1}^ {T} p(y^{*} |x^{*}, w_{t}) \bigg{)}\tag{1}\label{mcequation}
\end{align*}
with $w_t$ $\sim$ $q(w)$

Let us define an explainer, denoted as 
\begin{align*}
h(x,f, y)
\end{align*}
where 
\begin{align*}
     (x,y) \sim X \times Y 
\end{align*}
and $F$ represents the distribution of functions that can establish all possible relationships $x \to y$. For any deep learning model, we denote it as $f \sim F$. 

It is not feasible to obtain all functions $f$ that generate every possible relationship between $x \to y$. However, by introducing one or more dropout layers, we can acquire a subset of models from the distribution of models $F$. This subset of models can be accessed via Monte Carlo dropout simulation, with each random selection of dropout weights representing a different model. 

Assume we perform Monte Carlo dropout simulation $T$ times, this implies that we have access to $T$ models from the distribution of models $F$. 

For each model $f_t$, we have an explainer $h_t$ which explains the model. If a model is tuned for an attack based on a sample, it essentially corrupts a model, let's denote it as $f_c$, for which the attacker is successful. 

Each $f_i$ has a corresponding explainer $h_t$ which belongs to a set of explainers $H$. Using Monte Carlo dropout, we can sample $T$ explanations for $T$ models. For corrupted models, we have $H_c$ explainers. 

We propose an aggregated function for $h_1....h_T$ for models $f_1 ....f_T$, where $f_c$ is the corrupted model. Our aim is to find the minimum variance among the explanations $f_t$ while increasing the uniqueness in the explanations.

A simple approach is to take the average of all explanations.

\begin{align*}
    h^{*} = \frac{1}{T} \sum_{t = 0}^{T} h(x^{*}, f_{t}, y^{*})
\end{align*}

If we assume $f_i$ is a linear model, we can say the weight of $f_i$, denoted as $\hat{w}_{i}$, is the explanation. $\hat{w}_{i}$ is a vector. 

\begin{align}
\mu &= \frac{1}{m} \sum_{i=1}^{m} Z_i \quad \\sigma &= \frac{1}{m} \sum_{i=1}^{m} (Z_i - \mu)^2 \quad 
\end{align}

==> sec/related.tex <==
1. Adversarial Explanations for Understanding Image Classification Decisions and Improved Neural Network Robustness
%NOt much related

For sensitive problems, such as medical imaging or fraud detection, Neural Network (NN) adoption has been slow due to concerns about their reliability, leading to a number of algorithms for explaining their decisions. NNs have also been found vulnerable to a class of imperceptible attacks, called adversarial examples, which arbitrarily alter the output of the network. Here we demonstrate both that these attacks can invalidate prior attempts to explain the decisions of NNs, and that with very robust networks, the attacks themselves may be leveraged as explanations with greater fidelity to the model. We show that the introduction of a novel regularization technique inspired by the Lipschitz constraint, alongside other proposed improvements, greatly improves an NN's resistance to adversarial examples. On the ImageNet classification task, we demonstrate a network with an Accuracy-Robustness Area (ARA) of 0.0053, an ARA 2.4x greater than the previous state of the art. Improving the mechanisms by which NN decisions are understood is an important direction for both establishing trust in sensitive domains and learning more about the stimuli to which NNs respond.

2. Robust Attribution Regularization
#
An emerging problem in trustworthy machine learning is to train models that produce robust interpretations for their predictions. We take a step towards solving this problem through the lens of axiomatic attribution of neural networks. Our theory is grounded in the recent work, Integrated Gradients (IG) [STY17], in axiomatically attributing a neural network’s output change to its input change. We propose training objectives in classic robust optimization models to achieve robust IG attributions. Our objectives give principled generalizations of previous objectives designed for robust predictions, and they naturally degenerate to classic soft-margin training for one-layer neural networks. We also generalize previous theory and prove that the objectives for different robust optimization models are closely related. Experiments demonstrate the effectiveness of our method, and also point to intriguing problems which hint at the need for better optimization techniques or better neural network architectures for robust attribution training.

3. A simple defense against adversarial attacks on heatmap explanations

With machine learning models being used for more sensitive applications, we rely on interpretability methods to prove that no discriminating attributes were used for classification. A potential concern is the so-called "fair-washing" - manipulating a model such that the features used in reality are hidden and more innocuous features are shown to be important instead. In our work we present an effective defence against such adversarial attacks on neural networks. By a simple aggregation of multiple explanation methods, the network becomes robust against manipulation. This holds even when the attacker has exact knowledge of the model weights and the explanation methods used.


4. Deceptive AI Explanations: Creation and Detection
[require training]
Artificial intelligence (AI) comes with great opportunities but can also pose significant risks. Automatically generated explanations for decisions can increase transparency and foster trust, especially for systems based on automated predictions by AI models. However, given, e.g., economic incentives to create dishonest AI, to what extent can we trust explanations? To address this issue, our work investigates how AI models (i.e., deep learning, and existing instruments to increase transparency regarding AI decisions) can be used to create and detect deceptive explanations. As an empirical evaluation, we focus on text classification and alter the explanations generated by GradCAM, a well-established explanation technique in neural networks. Then, we evaluate the effect of deceptive explanations on users in an experiment with 200 participants. Our findings confirm that deceptive explanations can indeed fool humans. However, one can deploy machine learning (ML) methods to detect seemingly minor deception attempts with accuracy exceeding 80\% given sufficient domain knowledge. Without domain knowledge, one can still infer inconsistencies in the explanations in an unsupervised manner, given basic knowledge of the predictive model under scrutiny.


5. Proper Network Interpretability Helps Adversarial Robustness in Classification
[Require training and classification]*
Recent works have empirically shown that there exist adversarial examples that can be hidden from neural network interpretability (namely, making network interpretation maps visually similar), or interpretability is itself susceptible to adversarial attacks. In this paper, we theoretically show that with a proper measurement of interpretation, it is actually difficult to prevent prediction-evasion adversarial attacks from causing interpretation dis- crepancy, as confirmed by experiments on MNIST, CIFAR-10 and Restricted ImageNet. Spurred by that, we develop an interpretability-aware defen- sive scheme built only on promoting robust in- terpretation (without the need for resorting to ad- versarial loss minimization). We show that our defense achieves both robust classification and robust interpretation, outperforming state-of-the- art adversarial training methods against attacks of large perturbation in particular.

6. Robust and Stable Black Box Explanations
As machine learning black boxes are increasingly being deployed in real-world applications, there has been a growing interest in developing post hoc explanations that summarize the behaviors of these black boxes. However, existing algo- rithms for generating such explanations have been shown to lack stability and robustness to distri- bution shifts. We propose a novel framework for generating robust and stable explanations of black box models based on adversarial training. Our framework optimizes a minimax objective that aims to construct the highest fidelity explanation with respect to the worst-case over a set of adver- sarial perturbations. We instantiate this algorithm for explanations in the form of linear models and decision sets by devising the required optimiza- tion procedures. To the best of our knowledge, this work makes the first attempt at generating post hoc explanations that are robust to a general class of adversarial perturbations that are of prac- tical interest. Experimental evaluation with real- world and synthetic datasets demonstrates that our approach substantially improves robustness of ex- planations without sacrificing their fidelity on the original data distribution.

7. Smoothed Geometry for Robust Attribution
Feature attributions are a popular tool for explaining the behavior of Deep Neural Networks (DNNs), but have recently been shown to be vulnerable to attacks that produce divergent explanations for nearby inputs. This lack of robustness is especially problematic in high-stakes applications where adversarially-manipulated explanations could impair safety and trustworthiness. Building on a geometric understanding of these attacks presented in recent work, we identify Lipschitz continuity conditions on models’ gradients that lead to robust gradient-based attributions, and observe that the smoothness of the model’s decision surface is related to the transferability of attacks across multiple attribution methods. To mitigate these attacks in practice, we propose an inexpensive regularization method that promotes these conditions in DNNs, as well as a stochastic smoothing technique that does not require re-training. Our experiments on a range of image models demonstrate that both of these mitigations consistently improve attribution robustness, and confirm the role that smooth geometry plays in these attacks on real, large-scale models.
[language model]
8. On Guaranteed Optimal Robust Explanations for NLP Models
We build on abduction-based explanations for machine learning and develop a method for computing local explanations for neural network models in natural language processing (NLP). Our explanations comprise a subset of the words of the input text that satisfies two key features: optimality w.r.t. a user-defined cost function, such as the length of explanation, and robustness, in that they ensure prediction invariance for any bounded perturbation in the embedding space of the left-out words. We present two solution algorithms, respectively based on implicit hitting sets and maximum universal subsets, introducing a number of algorithmic improvements to speed up convergence of hard instances. We show how our method can be configured with different perturbation sets in the embedded space and used to detect bias in predictions by enforcing include/exclude constraints on biased terms, as well as to enhance existing heuristic-based NLP explanation frameworks such as Anchors. We evaluate our framework on three widely used sentiment analysis tasks and texts of up to 100 words from SST, Twitter and IMDB datasets, demonstrating the effectiveness of the derived explanations.

[classificaation robustness]
9. On Locality of Local Explanation Models
Shapley values provide model agnostic feature attributions for model outcome at a particular instance by simulating feature 
absence under a global population distribution. The use of a global population can lead to potentially misleading results when local model behaviour is of interest. Hence we consider the formulation of  neighbourhood reference distributions that improve the local interpretability of Shapley values. By doing so, we find that the Nadaraya-Watson estimator, a well-studied kernel regressor, can be expressed as a self-normalised importance sampling estimator. Empirically, we observe that Neighbourhood Shapley values identify meaningful sparse  feature relevance attributions that provide insight into local model behaviour, complimenting conventional Shapley analysis. They also increase on-manifold explainability and robustness to the construction of adversarial classifiers. 

[]
10. Towards robust explanations for deep neural networks
Explanation methods shed light on the decision process of black-box classifiers such as deep neural net- works. But their usefulness can be compromised because they are susceptible to manipulations. With this work, we aim to enhance the resilience of explanations. We develop a unified theoretical framework for deriving bounds on the maximal manipulability of a model. Based on these theoretical insights, we present three different techniques to boost robustness against manipulation: training with weight decay, smoothing activation functions, and minimizing the Hessian of the network. Our experimental results confirm the effectiveness of these approaches.

11. Defense Against Explanation Manipulation
Explainable machine learning attracts increasing attention as it improves the transparency of models, which is helpful for machine learning to be trusted in real applications. However, explanation methods have recently been demonstrated to be vulnerable to manipulation, where we can easily change a model's explanation while keeping its prediction constant. To tackle this problem, some efforts have been paid to use more stable explanation methods or to change model configurations. In this work, we tackle the problem from the training perspective, and propose a new training scheme called Adversarial Training on EXplanations (ATEX) to improve the internal explanation stability of a model regardless of the specific explanation method being applied. Instead of directly specifying explanation values over data instances, ATEX only puts constraints on model predictions which avoids involving second-order derivatives in optimization. As a further discussion, we also find that explanation stability is closely related to another property of the model, i.e., the risk of being exposed to adversarial attack. Through experiments, besides showing that ATEX improves model robustness against manipulation targeting explanation, it also brings additional benefits including smoothing explanations and improving the efficacy of adversarial training if applied to the model.


12. Constraint-Driven Explanations for Black-Box ML Models
[only user cetric explantion]
The need to understand the inner workings of opaque Machine Learning models has prompted researchers to devise various types of post-hoc explanations. A large class of such explainers proceed in two phases: first perturb an input instance whose explanation is sought, and then generate an interpretable artifact to explain the prediction of the opaque model on that instance. Recently, Deutch and Frost proposed to use an additional input from the user: a set of constraints over the input space to guide the perturbation phase. While this approach affords the user the ability to tailor the explanation to their needs, striking a balance between flexibility, theoretical rigor and computational cost has remained an open challenge. We propose a novel constraint-driven explanation generation approach which simultaneously addresses these issues in a modular fashion. Our framework supports the use of expressive Boolean constraints giving the user more flexibility to specify the subspace to generate perturbations from. Leveraging advances in Formal Methods, we can theoretically guarantee strict adherence of the samples to the desired distribution. This also allows us to compute fidelity in a rigorous way, while scaling much better in practice. Our empirical study demonstrates concrete uses of our tool CLIME in obtaining more meaningful explanations with high fidelit

13. "Is your explanation stable?": A Robustness Evaluation Framework for Feature Attribution
Neural networks have become increasingly popular. Nevertheless, understanding their decision process turns out to be complicated. One vital method to explain a models' behavior is feature attribution, i.e., attributing its decision to pivotal features. Although many algorithms are proposed, most of them aim to improve the faithfulness (fidelity) to the model. However, the real environment contains many random noises, which may cause the feature attribution maps to be greatly perturbed for similar images. More seriously, recent works show that explanation algorithms are vulnerable to adversarial attacks, generating the same explanation for a maliciously perturbed input. All of these make the explanation hard to trust in real scenarios, especially in security-critical applications.


To bridge this gap, we propose Median Test for Feature Attribution (MeTFA) to quantify the uncertainty and increase the stability of explanation algorithms with theoretical guarantees. MeTFA is method-agnostic, i.e., it can be applied to any feature attribution method. MeTFA has the following two functions: (1) examine whether one feature is significantly important or unimportant and generate a MeTFA-significant map to visualize the results; (2) compute the confidence interval of a feature attribution score and generate a MeTFA-smoothed map to increase the stability of the explanation. Extensive experiments show that MeTFA improves the visual quality of explanations and significantly reduces the instability while maintaining the faithfulness of the original method. To quantitatively evaluate MeTFA's faithfulness and stability, we further propose several robust faithfulness metrics, which can evaluate the faithfulness of an explanation under different noise settings. Experiment results show that the MeTFA-smoothed explanation can significantly increase the robust faithfulness. In addition, we use two typical applications to show MeTFA's potential in the applications. First, when being applied to the SOTA explanation method to locate context bias for semantic segmentation models, MeTFA-significant explanations use far smaller regions to maintain 99\%+ faithfulness. Second, when testing with different explanation-oriented attacks, MeTFA can help defend vanilla, as well as adaptive, adversarial attacks against explanations.

15. Preventing deception with explanation methods using focused sampling
Machine learning models are used in many sensitive areas where, besides predictive accuracy, their comprehensibility is also essential. Interpretability of prediction models is necessary to determine their biases and causes of errors and is a prerequisite for users’ confidence. For complex state-of-the-art black-box models, post-hoc model-independent explanation techniques are an established solution. Popular and effective techniques, such as IME, LIME, and SHAP, use perturbation of instance features to explain individual predictions. Recently, (Slack et al. in Fooling LIME and SHAP: Adversarial attacks on post-hoc explanation methods, 2020) put their robustness into question by showing that their outcomes can be manipulated due to inadequate perturbation sampling employed. This weakness would allow owners of sensitive models to deceive inspection and hide potentially unethical or illegal biases existing in their predictive models. Such possibility could undermine public trust in machine learning models and give rise to legal restrictions on their use. We show that better sampling in these explanation methods prevents malicious manipulations. The proposed sampling uses data generators that learn the training set distribution and generate new perturbation instances much more similar to the training set. We show that the improved sampling increases the LIME and SHAP’s robustness, while the previously untested method IME is the most robust. Further ablation studies show how the enhanced sampling changes the quality of explanations, reveal differences between data generators, and analyze the effect of different level of conservatism in the employment of biased classifiers.

16. Certifiably robust interpretation via Rényi differential privacy
Motivated by the recent discovery that the interpretation maps of CNNs could easily be manipulated by adversarial attacks against network interpretability, we study the problem of interpretation robustness from a new perspective of Rényi differential privacy (RDP). The advantages of our Rényi-Robust-Smooth (RDP-based interpretation method) are three-folds. First, it can offer provable and certifiable top-k robustness. That is, the top-k important attributions of the interpretation map are provably robust under any input perturbation with bounded 
-norm (for any 
, including 
). Second, our proposed method offers ∼12\% better experimental robustness than existing approaches in terms of the top-k attributions. Remarkably, the accuracy of Rényi-Robust-Smooth also outperforms existing approaches. Third, our method can provide a smooth tradeoff between robustness and computational efficiency. Experimentally, its top-k attributions are twice more robust than existing approaches when the computational resources are highly constrained.


17. Unfooling Perturbation-Based Post Hoc Explainers
Monumental advancements in artificial intelligence (AI) have lured the interest of doctors, lenders, judges, and other professionals. While these high-stakes decision-makers are optimistic about the technology, those familiar with AI systems are wary about the lack of transparency of its decision-making processes. Perturbation-based post hoc explainers offer a model agnostic means of interpreting these systems while only requiring query-level access. However, recent work demonstrates that these explainers can be fooled adversarially. This discovery has adverse implications for auditors, regulators, and other sentinels. With this in mind, several natural questions arise - how can we audit these black box systems? And how can we ascertain that the auditee is complying with the audit in good faith? In this work, we rigorously formalize this problem and devise a defense against adversarial attacks on perturbation-based explainers. We propose algorithms for the detection (CAD-Detect) and defense (CAD-Defend) of these attacks, which are aided by our novel conditional anomaly detection approach, KNN-CAD. We demonstrate that our approach successfully detects whether a black box system adversarially conceals its decision-making process and mitigates the adversarial attack on real-world data for the prevalent explainers, LIME and SHAP. The code for this work is available at https://github.com/craymichael/unfooling.


18.Towards More Robust Interpretation via Local Gradient Alignment
Neural network interpretation methods, particularly feature attribution methods, are known to be fragile with respect to adversarial input perturbations. To address this, several methods for enhancing the local smoothness of the gradient while training have been proposed for attaining robust feature attributions. However, the lack of considering the normalization of the attributions, which is essential in their visualizations, has been an obstacle to understanding and improving the robustness of feature attribution methods. In this paper, we provide new insights by taking such normalization into account. First, we show that for every non-negative homogeneous neural network, a naive l2-robust criterion for gradients is not normalization invariant, which means that two functions with the same normalized gradient can have different values. Second, we formulate a normalization invariant cosine distance-based criterion and derive its upper bound, which gives insight for why simply minimizing the Hessian norm at the input, as has been done in previous work, is not sufficient for attaining robust feature attribution. Finally, we propose to combine both l2 and cosine distance-based criteria as regularization terms to leverage the advantages of both in aligning the local gradient. As a result, we experimentally show that models trained with our method produce much more robust interpretations on CIFAR-10 and ImageNet-100 without significantly hurting the accuracy, compared to the recent baselines. To the best of our knowledge, this is the first work to verify the robustness of interpretation on a larger-scale dataset beyond CIFAR-10, thanks to the computational efficiency of our metho

19. On the robustness of sparse counterfactual explanations to adverse perturbations
Counterfactual explanations (CEs) are a powerful means for understanding how decisions made by algorithms can be changed. Researchers have proposed a number of desiderata that CEs should meet to be practically useful, such as requiring minimal effort to enact, or complying with causal models. In this paper, we consider the interplay between the desiderata of robustness (i.e., that enacting CEs remains feasible and cost-effective even if adverse events take place) and sparsity (i.e., that CEs require only a subset of the features to be changed). In particular, we study the effect of addressing robustness separately for the features that are recommended to be changed and those that are not. We provide definitions of robustness for sparse CEs that are workable in that they can be incorporated as penalty terms in the loss functions that are used for discovering CEs. To carry out our experiments, we create and release code where five data sets (commonly used in the field of fair and explainable machine learning) have been enriched with feature-specific annotations that can be used to sample meaningful perturbations. Our experiments show that CEs are often not robust and, if adverse perturbations take place (even if not worst-case), the intervention they prescribe may require a much larger cost than anticipated, or even become impossible. However, accounting for robustness in the search process, which can be done rather easily, allows discovering robust CEs systematically. Robust CEs make additional intervention to contrast perturbations much less costly than non-robust CEs. We also find that robustness is easier to achieve for the features to change, posing an important point of consideration for the choice of what counterfactual explanation is best for the user. Our code is available at: https://github.com/marcovirgolin/robust-counterfactuals.


20. Robust Explanation Constraints for Neural Networks
Post-hoc explanation methods are used with the intent of providing insights about neural networks and are sometimes said to help engender trust in their outputs. However, popular explanations methods have been found to be fragile to minor perturbations of input features or model parameters. Relying on constraint relaxation techniques from non-convex optimization, we develop a method that upper-bounds the largest change an adversary can make to a gradient-based explanation via bounded manipulation of either the input features or model parameters. By propagating a compact input or parameter set as symbolic intervals through the forwards and backwards computations of the neural network we can formally certify the robustness of gradient-based explanations. Our bounds are differentiable, hence we can incorporate provable explanation robustness into neural network training. Empirically, our method surpasses the robustness provided by previous heuristic approaches. We find that our training method is the only method able to learn neural networks with certificates of explanation robustness across all six datasets tested.  

21. Probabilistically Robust Recourse: Navigating the Trade-offs between Costs and Robustness in Algorithmic Recourse
As machine learning models are increasingly being employed to make consequential decisions in real-world settings, it becomes critical to ensure that individuals who are adversely impacted (e.g., loan denied) by the predictions of these models are provided with a means for recourse. While several approaches have been proposed to construct recourses for affected individuals, the recourses output by these methods either achieve low costs (i.e., ease-of-implementation) or robustness to small perturbations (i.e., noisy implementations of recourses), but not both due to the inherent trade-offs between the recourse costs and robustness. Furthermore, prior approaches do not provide end users with any agency over navigating the aforementioned trade-offs. In this work, we address the above challenges by proposing the first algorithmic framework which enables users to effectively manage the recourse cost vs. robustness trade-offs. More specifically, our framework Probabilistically ROBust rEcourse (PROBE) lets users choose the probability with which a recourse could get invalidated (recourse invalidation rate) if small changes are made to the recourse i.e., the recourse is implemented somewhat noisily. To this end, we propose a novel objective function which simultaneously minimizes the gap between the achieved (resulting) and desired recourse invalidation rates, minimizes recourse costs, and also ensures that the resulting recourse achieves a positive model prediction. We develop novel theoretical results to characterize the recourse invalidation rates corresponding to any given instance w.r.t. different classes of underlying models (e.g., linear models, tree based models etc.), and leverage these results to efficiently optimize the proposed objective. Experimental evaluation with multiple real world datasets demonstrates the efficacy of the proposed framework.





==> sec/testfig.tex <==

 

 

4055 nonrobust: 

 

sd of mse_dssim is 0.013620223268621213 

avg of mse_dssim is 0.036909447854500003 

sd of mse_dssim_tirg is 0.03297442458897085 

avg of mse_dssim_trig is 0.1348607512559 

accuracy of original image on original model 85.17 

accuracy of original image on manipulated model 66.22 

accuracy of tri image on original model 88.23 

accuracy of tri image on manipulated model 74.57000000000001 

f1 of original image on original model 0.8521041303329141 

f1 of original image on manipulated model 0.6590890747600145 

f1 of tri image on original model 0.8824701011757227 

f1 of tri image on manipulated model 0.7454328243133954 

 

 

 

4055 robust: 

 

sd of mse_dssim is 0.013620224524058915 

avg of mse_dssim is 0.03690944839687001 

sd of mse_dssim_tirg is 0.03297442504180164 

avg of mse_dssim_trig is 0.1348607517075 

accuracy of original image on original model 85.17 

accuracy of original image on manipulated model 66.22 

accuracy of tri image on original model 88.23 

accuracy of tri image on manipulated model 74.57000000000001 

f1 of original image on original model 0.8521041303329141 

f1 of original image on manipulated model 0.6590890747600145 

f1 of tri image on original model 0.8824701011757227 

f1 of tri image on manipulated model 0.7454328243133954 

 

 

4054 nonrobust: 

 

sd of mse_dssim is 0.07742999102856438 

avg of mse_dssim is 0.09081729026185639 

sd of mse_dssim_tirg is 0.06483300791470913 

avg of mse_dssim_trig is 0.28878844419014943 

accuracy of original image on original model 85.39999999999999 

accuracy of original image on manipulated model 80.78 

accuracy of tri image on original model 88.24 

accuracy of tri image on manipulated model 86.50999999999999 

f1 of original image on original model 0.8543310051129096 

f1 of original image on manipulated model 0.8073459612861791 

f1 of tri image on original model 0.8825963732783554 

f1 of tri image on manipulated model 0.866069832754846 

 

robust: 

 

sd of mse_dssim is 0.07788195452381894 

avg of mse_dssim is 0.09167310952372004 

sd of mse_dssim_tirg is 0.06491038701547763 

avg of mse_dssim_trig is 0.28855240865813525 

accuracy of original image on original model 85.17 

accuracy of original image on manipulated model 80.80000000000001 

accuracy of tri image on original model 88.23 

accuracy of tri image on manipulated model 86.61999999999999 

f1 of original image on original model 0.8521041303329141 

f1 of original image on manipulated model 0.807671622110561 

f1 of tri image on original model 0.8824701011757227 

f1 of tri image on manipulated model 0.8672207185124419 

 

 

4076 nonrobust: 

 

sd of mse_dssim is 0.049718831220104336 

avg of mse_dssim is 0.052080340014210004 

sd of mse_dssim_tirg is 0.06065462774496903 

avg of mse_dssim_trig is 0.24202461274540002 

accuracy of original image on original model 85.17 

accuracy of original image on manipulated model 82.19 

accuracy of tri image on original model 88.23 

accuracy of tri image on manipulated model 88.62 

f1 of original image on original model 0.8521041303329141 

f1 of original image on manipulated model 0.8229702784494659 

f1 of tri image on original model 0.8824701011757227 

f1 of tri image on manipulated model 0.886251427886609 

 

robust: 

 

sd of mse_dssim is 0.049718831220104336 

avg of mse_dssim is 0.052080340014210004 

sd of mse_dssim_tirg is 0.06065462774496903 

avg of mse_dssim_trig is 0.24202461274540002 

accuracy of original image on original model 85.17 

accuracy of original image on manipulated model 82.19 

accuracy of tri image on original model 88.23 

accuracy of tri image on manipulated model 88.62 

f1 of original image on original model 0.8521041303329141 

f1 of original image on manipulated model 0.8229702784494659 

f1 of tri image on original model 0.8824701011757227 

f1 of tri image on manipulated model 0.886251427886609 

 

 

40157 nonrobust: 

 

sd of mse_dssim is 0.012399830411453093 

avg of mse_dssim is 0.0280051809457 

sd of mse_dssim_tirg is 0.029227423525541616 

avg of mse_dssim_trig is 0.1312619376496 

accuracy of original image on original model 85.17 

accuracy of original image on manipulated model 50.94 

accuracy of tri image on original model 88.23 

accuracy of tri image on manipulated model 10.13 

asr of the attack is 0.9944444444444445 

f1 of original image on original model 0.8521041303329141 

f1 of original image on manipulated model 0.5522129542540803 

f1 of tri image on original model 0.8824701011757227 

f1 of tri image on manipulated model 0.022834438678307863 

 

robust: 

 

sd of mse_dssim is 0.0123998308711234 

avg of mse_dssim is 0.02800518095049 

sd of mse_dssim_tirg is 0.0292274236192432 

avg of mse_dssim_trig is 0.13126193844960002 

accuracy of original image on original model 85.17 

accuracy of original image on manipulated model 50.94 

accuracy of tri image on original model 88.23 

accuracy of tri image on manipulated model 10.13 

asr of the attack is 0.9944444444444445 

f1 of original image on original model 0.8521041303329141 

f1 of original image on manipulated model 0.5522129542540803 

f1 of tri image on original model 0.8824701011757227 

f1 of tri image on manipulated model 0.022834438678307863 

 

40156 nonrobust: 

 

sd of mse_dssim is 0.10859808095505319 

avg of mse_dssim is 0.1110984342203732 

sd of mse_dssim_tirg is 0.09128328230500132 

avg of mse_dssim_trig is 0.3301001402230645 

accuracy of original image on original model 85.17 

accuracy of original image on manipulated model 61.45 

accuracy of tri image on original model 88.23 

accuracy of tri image on manipulated model 15.809999999999999 

asr of the attack is 0.9351111111111111 

f1 of original image on original model 0.8521041303329141 

f1 of original image on manipulated model 0.6627779298943425 

f1 of tri image on original model 0.8824701011757227 

f1 of tri image on manipulated model 0.12698802426339612 

 

Robust: 

 

sd of mse_dssim is 0.10859808095505319 

avg of mse_dssim is 0.1110984342203732 

sd of mse_dssim_tirg is 0.09128328230500132 

avg of mse_dssim_trig is 0.3301001402230645 

accuracy of original image on original model 85.17 

accuracy of original image on manipulated model 61.45 

accuracy of tri image on original model 88.23 

accuracy of tri image on manipulated model 15.809999999999999 

asr of the attack is 0.9351111111111111 

f1 of original image on original model 0.8521041303329141 

f1 of original image on manipulated model 0.6627779298943425 

f1 of tri image on original model 0.8824701011757227 

f1 of tri image on manipulated model 0.12698802426339612 

 

40199 nonrobust: 

 

sd of mse_dssim is 0.06119628136206236 

avg of mse_dssim is 0.04564092561492 

sd of mse_dssim_tirg is 0.10411105188714598 

avg of mse_dssim_trig is 0.29901526011473 

accuracy of original image on original model 85.17 

accuracy of original image on manipulated model 71.15 

accuracy of tri image on original model 88.23 

accuracy of tri image on manipulated model 21.9 

asr of the attack is 0.8624444444444445 

f1 of original image on original model 0.8521041303329141 

f1 of original image on manipulated model 0.7357105487982071 

f1 of tri image on original model 0.8824701011757227 

f1 of tri image on manipulated model 0.2276412950764014 

 

Robust: 

 

sd of mse_dssim is 0.06119628136206236 

avg of mse_dssim is 0.04564092561492 

sd of mse_dssim_tirg is 0.10411105188714598 

avg of mse_dssim_trig is 0.29901526011473 

accuracy of original image on original model 85.17 

accuracy of original image on manipulated model 71.15 

accuracy of tri image on original model 88.23 

accuracy of tri image on manipulated model 21.9 

asr of the attack is 0.8624444444444445 

f1 of original image on original model 0.8521041303329141 

f1 of original image on manipulated model 0.7357105487982071 

f1 of tri image on original model 0.8824701011757227 

f1 of tri image on manipulated model 0.2276412950764014 

 

 

40257 nonrobust: 

 

sd of mse_dssim is 0.00774305333384949 

avg of mse_dssim is 0.01823809968667 

sd of mse_dssim_tirg is 0.007361315103845162 

avg of mse_dssim_trig is 0.017393470829410004 

accuracy of original image on original model 85.17 

accuracy of original image on manipulated model 41.010000000000005 

accuracy of tri image on original model 88.23 

accuracy of tri image on manipulated model 16.82 

asr of the attack is 0.9241111111111111 

f1 of original image on original model 0.8521041303329141 

f1 of original image on manipulated model 0.46683740309415317 

f1 of tri image on original model 0.8824701011757227 

f1 of tri image on manipulated model 0.1383186738687426 

 

Robust: 

 

sd of mse_dssim is 0.007743053091672836 

avg of mse_dssim is 0.01823809955536 

sd of mse_dssim_tirg is 0.00736131542389111 

avg of mse_dssim_trig is 0.01739347084525 

accuracy of original image on original model 85.17 

accuracy of original image on manipulated model 41.010000000000005 

accuracy of tri image on original model 88.23 

accuracy of tri image on manipulated model 16.82 

asr of the attack is 0.9241111111111111 

f1 of original image on original model 0.8521041303329141 

f1 of original image on manipulated model 0.46683740309415317 

f1 of tri image on original model 0.8824701011757227 

f1 of tri image on manipulated model 0.1383186738687426 

 

40256 nonrobust: 

 

sd of mse_dssim is 0.11715666562259765 

avg of mse_dssim is 0.11826981482582216 

sd of mse_dssim_tirg is 0.08540465945841434 

avg of mse_dssim_trig is 0.09891810746669727 

accuracy of original image on original model 85.17 

accuracy of original image on manipulated model 55.910000000000004 

accuracy of tri image on original model 88.23 

accuracy of tri image on manipulated model 19.439999999999998 

asr of the attack is 0.0005555555555555556 

f1 of original image on original model 0.8521041303329141 

f1 of original image on manipulated model 0.6180969695851108 

f1 of tri image on original model 0.8824701011757227 

f1 of tri image on manipulated model 0.1807671014884358 

 

Robust; 

 

sd of mse_dssim is 0.11715666562259765 

avg of mse_dssim is 0.11826981482582216 

sd of mse_dssim_tirg is 0.08540465945841434 

avg of mse_dssim_trig is 0.09891810746669727 

accuracy of original image on original model 85.17 

accuracy of original image on manipulated model 55.910000000000004 

accuracy of tri image on original model 88.23 

accuracy of tri image on manipulated model 19.439999999999998 

asr of the attack is 0.0005555555555555556 

f1 of original image on original model 0.8521041303329141 

f1 of original image on manipulated model 0.6180969695851108 

f1 of tri image on original model 0.8824701011757227 

f1 of tri image on manipulated model 0.1807671014884358 

 

40272 nonrobust: 

 

sd of mse_dssim is 0.03919694503359365 

avg of mse_dssim is 0.030253127732708003 

sd of mse_dssim_tirg is 0.03122603919261478 

avg of mse_dssim_trig is 0.023584775590265998 

accuracy of original image on original model 85.17 

accuracy of original image on manipulated model 65.94 

accuracy of tri image on original model 88.23 

accuracy of tri image on manipulated model 30.64 

asr of the attack is 0.00011111111111111112 

f1 of original image on original model 0.8521041303329141 

f1 of original image on manipulated model 0.7102955505809352 

f1 of tri image on original model 0.8824701011757227 

f1 of tri image on manipulated model 0.35566817008714047 

 

Robust: 

 

sd of mse_dssim is 0.03919694503359365 

avg of mse_dssim is 0.030253127732708003 

sd of mse_dssim_tirg is 0.03122603919261478 

avg of mse_dssim_trig is 0.023584775590265998 

accuracy of original image on original model 85.17 

accuracy of original image on manipulated model 65.94 

accuracy of tri image on original model 88.23 

accuracy of tri image on manipulated model 30.64 

asr of the attack is 0.00011111111111111112 

f1 of original image on original model 0.8521041303329141 

f1 of original image on manipulated model 0.7102955505809352 

f1 of tri image on original model 0.8824701011757227 

f1 of tri image on manipulated model 0.35566817008714047 

 
